Neural Chronos ODE: Unveiling Temporal Patterns and Forecasting Future and Past Trends in Time Series Data

This work introduces Neural Chronos Ordinary Differential Equations (Neural CODE), a deep neural network architecture that fits a continuous-time ODE dynamics for predicting the chronology of a system both forward and backward in time. To train the model, we solve the ODE as an initial value problem and a final value problem, similar to Neural ODEs. We also explore two approaches to combining Neural CODE with Recurrent Neural Networks by replacing Neural ODE with Neural CODE (CODE-RNN), and incorporating a bidirectional RNN for full information flow in both time directions (CODE-BiRNN), and variants with other update cells namely GRU and LSTM: CODE-GRU, CODE-BiGRU, CODE-LSTM, CODE-BiLSTM. Experimental results demonstrate that Neural CODE outperforms Neural ODE in learning the dynamics of a spiral forward and backward in time, even with sparser data. We also compare the performance of CODE-RNN/-GRU/-LSTM and CODE-BiRNN/-BiGRU/-BiLSTM against ODE-RNN/-GRU/-LSTM on three real-life time series data tasks: imputation of missing data for lower and higher dimensional data, and forward and backward extrapolation with shorter and longer time horizons. Our findings show that the proposed architectures converge faster, with CODE-BiRNN/-BiGRU/-BiLSTM consistently outperforming the other architectures on all tasks.

==> 6-Limitations.tex <==
\section{Limitations} \label{sec:limitations}

% \noindent \textbf{Ordinary differential equations can be too simple.} If the data being modelled is noisy or presents high variance, an ODE may not be able to fit the underlying dynamics of the system well enough. 

% \noindent \textbf{Nonlinear ODEs can be erratic.} The adjusted ODE is given by a NN and its form depends on the chosen activation functions. When all activation functions are linear, then the NN adjusts a linear ODE, if at least one is a nonlinear function, then the NN builds a nonlinear ODE. 
% Nonlinear ODEs often have points where the solution is undefined or not well behaved. These singularities can make it difficult to solve the ODE numerically, because the numerical methods used to approximate the solution may not be accurate near the singularities \citepp{chapraNumericalMethodsEngineers2021}.
% Although nonlinear ODEs are challenging to solve, they can model rich and complex behaviour.

% \noindent \textbf{ODEs adjusted by Neural CODE may not accurately model real-world systems.} The behaviour of a physical system at a given point in time may depend on the events that occurred leading up to that point and therefore the behaviour of the system may be different depending on whether it is moving forward or backward in time. By adjusting an ODE by forcing it to solve an IVP and FVP, Neural CODE may not accurately capture the underlying dynamics of the data, which can make it tricky to use the ODE to understand s system's behaviour where the direction of time is important (where cause and effect are important). 


% \noindent \textbf{Neural CODE assumes the dimension of the input and output is the same.} Neural ODEs have been used for tasks such as image classification, where the input (considered to be the first time step) is a vector with the pixel values of the image while the expected output (value at the last time step) is the label of the image, that can be given as a vector with the length of the number of possible labels \citepp{chenNeuralOrdinaryDifferential2019}. Also, it is usual to do regression with different input and output dimensions.
% Neural CODE does a double pass through time, meaning that it solves the ODE forwards by using the first step data point as initial value (IVP) and backwards by using the last time step data point as final value (FVP). This makes it impossible to directly use inputs and outputs that are not of the same dimension, since the NN that adjusts the ODE has a fixed size input and output layer that must have the same dimension. 


% \noindent \textbf{Neural CODE has higher computational cost.} Neural CODE uses a numerical method to solve an ODE twice, one for the initial value problem and another for the final value problem. To optimize Neural CODE, the total loss function has two terms and is given by the sum of the losses of each problem. So the adjoint method is also used twice, one for each problem. When compared with Neural ODE, Neural CODE has twice the computational cost. 


\textbf{Ordinary differential equations may be too simplistic:}

Ordinary differential equations (ODEs) may sometimes be too simplistic. When dealing with noisy or highly variable data, an ODE might struggle to accurately capture the underlying dynamics of the system.

\textbf{Challenges of nonlinear ODEs:}

Nonlinear ODEs can exhibit erratic behavior. The structure of the adjusted ODE is determined by a NN, which relies on chosen activation functions. If all activation functions are linear, the NN adjusts a linear ODE; however, if at least one activation function is nonlinear, the NN constructs a nonlinear ODE. Nonlinear ODEs often contain undefined or poorly behaved solutions at certain points, making it challenging to solve them numerically. The presence of singularities near these points can compromise the accuracy of numerical approximation methods \citep{chapraNumericalMethodsEngineers2021}. Nonetheless, nonlinear ODEs have the ability to model intricate and complex behaviour.

\textbf{Limitations of Neural CODE for real-world systems:}

The adjustment of an ODE using Neural CODE, which forces the solution of IVPs and FVPs, may not accurately capture the underlying dynamics of real-world systems. The behaviour of a physical system at any given point in time can depend on past events, resulting in different behaviours when moving forward or backward in time. Consequently, the use of Neural CODE to understand systems where the direction of time is crucial (such as cause and effect relationships).

\textbf{Matching input and output dimensions with Neural CODE:}

Neural CODE assumes that the dimensions of the input and output are the same. For instance, in image classification tasks, the input (considered as the first time step) represents a vector of pixel values, while the output (at the last time step) corresponds to the image label, usually represented as a vector with a length equal to the number of possible labels \citep{chenNeuralOrdinaryDifferential2019}. Regression tasks may involve different input and output dimensions. Since Neural CODE performs a double pass through time, solving the ODE both forwards and backwards, it requires fixed-size input and output layers in the NN that adjusts the ODE. Consequently, directly using inputs and outputs of different dimensions is not straightforward.

\textbf{Computational cost of Neural CODE:}

Neural CODE incurs a higher computational cost compared to Neural ODE. It involves solving the ODE twice using a numerical method, once for the initial value problem and again for the final value problem. The optimisation of Neural CODE entails a total loss function consisting of two terms, which are the sum of losses for each problem. Consequently, the adjoint method is applied twice, once for each problem. As a result, Neural CODE approximately doubles the computational cost of Neural ODE.

==> trash/5-Autoencoder.tex <==
\subsection{Neural ODE Autoencoder}

\subsubsection*{Computational cost}

==> trash/6-Latent.tex <==
\subsection{The latent TBA ODE-RNN}



\begin{algorithm}[H]
\caption{The Latent TBA ODE-RNN. A Variational Autoencoder with a TBA ODE-RNN encoder and a Neural ODE decoder.}
\label{alg:latentODELSTM}
\begin{algorithmic}

\State \textbf{Input:} Data points and their timestamps $\{(x_i,t_i)\}_{i=1..N}$
\State $z'_0= \text{TBA ODE-RNN} (\{x_i\}_{i=1..N})$
\State $\mu, \sigma = g_\mu(z'_0),g_\sigma(z'_0)$
\State $z_0 \sim \mathcal{N}(\mu, \theta)$
\State $\{z_t\}_{0..N} = ODESolve(f_\theta,z_0,(t_0...t_N))$
\State $\tilde{x}_i =OutputNN(z_t)$ for all $i=1..N$, $t=1..N$
\State \textbf{Return:} $\{ \tilde{x}_i \}_{i=1..N}$

\end{algorithmic}
\end{algorithm}



\subsubsection*{Computational cost}

\subsection{The latent TBA ODE-BiRNN}



\begin{algorithm}[H]
\caption{The Latent TBA ODE-BiRNN. A Variational Autoencoder with a TBA ODE-BiRNN encoder and a Neural ODE decoder.}
\label{alg:latentODELSTM}
\begin{algorithmic}

\State \textbf{Input:} Data points and their timestamps $\{(x_i,t_i)\}_{i=1..N}$
\State $z'_0= \text{TBA ODE-BiRNN} (\{x_i\}_{i=1..N})$
\State $\mu, \sigma = g_\mu(z'_0),g_\sigma(z'_0)$
\State $z_0 \sim \mathcal{N}(\mu, \theta)$
\State $\{z_t\}_{0..N} = ODESolve(f_\theta,z_0,(t_0...t_N))$
\State $\tilde{x}_i =OutputNN(z_t)$ for all $i=1..N$, $t=1..N$
\State \textbf{Return:} $\{ \tilde{x}_i \}_{i=1..N}$

\end{algorithmic}
\end{algorithm}



\subsubsection*{Computational cost}
